Associated production of a Higgs boson decaying into bottom quarks and a weak vector boson decaying leptonically at NNLO in QCD

We present the calculation of next-to-next-to-leading order (NNLO) corrections in perturbative QCD for the production of a Higgs boson decaying into a pair of bottom quarks in association with a leptonically decaying weak vector boson: $\mathrm{pp} \to V \mathrm{H} + X \to \ell\bar{\ell}\;\mathrm{b\bar{b}} + X$. We consider the corrections to both the production and decay sub-processes, retaining a fully differential description of the final state including off-shell propagators of the Higgs and vector boson. The calculation is carried out using the antenna subtraction formalism and is implemented in the NNLOJET framework. Clustering and identification of $\mathrm{b}$-jets is performed with the flavour-$k_t$ algorithm and results for fiducial cross sections and distributions are presented for the LHC at $\sqrt{s}=13\;\text{TeV}$. We assess the residual theory uncertainty by varying the production and decay scales independently and provide scale uncertainty bands in our results, yielding percent-level accurate predictions for observables in this Higgs production mode computed at NNLO. Confronting a na\"ive perturbative expansion of the cross section against the customary re-scaling procedure to a fixed branching ratio reveals that starting from NNLO, the latter could be inadequate in estimating missing higher-order effects through scale variations.

==> fig.tex <==
\makeatletter

\newif\ifstartcompletesineup
\newif\ifendcompletesineup
\pgfkeys{
    /pgf/decoration/.cd,
    start up/.is if=startcompletesineup,
    start up=true,
    start up/.default=true,
    start down/.style={/pgf/decoration/start up=false},
    end up/.is if=endcompletesineup,
    end up=true,
    end up/.default=true,
    end down/.style={/pgf/decoration/end up=false}
}
\pgfdeclaredecoration{complete sines}{initial}
{
    \state{initial}[
        width=+0pt,
        next state=upsine,
        persistent precomputation={
            \ifstartcompletesineup
                \pgfkeys{/pgf/decoration automaton/next state=upsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5*\pgfdecoratedinputsegmentlength / (ceil(0.5* \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) )
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.499)
                    }
                \fi
            \else
                \pgfkeys{/pgf/decoration automaton/next state=downsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5* \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.4999)
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) )
                    }
                \fi
            \fi
            \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
        }] {}
    \state{downsine}[width=\pgfdecorationsegmentlength,next state=upsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
    }
    \state{upsine}[width=\pgfdecorationsegmentlength,next state=downsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
}
    \state{final}{}
}


\pgfdeclaredecoration{spring}{initial}
{
  \state{initial}[
    width=+0pt,
    next state=coil,
    persistent precomputation={
      \pgfmathsetmacro\matchinglength{
        (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) - \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) > 0.5
        ? (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (floor(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
        : (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
      }
      \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
    },
  ]{}
  \state{coil}[
    switch if less than=%
      0.5\pgfdecorationsegmentlength%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude to last,
    width=+\pgfdecorationsegmentlength,
  ]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{ 1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{ 2}}
    {\pgfpoint@oncoil{1    }{ 1    }{ 3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{ 4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{ 5}}
    {\pgfpoint@oncoil{2    }{ 0    }{ 6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{ 7}}
    {\pgfpoint@oncoil{1.555}{-1    }{ 8}}
    {\pgfpoint@oncoil{1    }{-1    }{ 9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}{}
}



\tikzset{
      % style to apply some styles to each segment of a path
      on each segment/.style={
        decorate,
        decoration={
          show path construction,
          moveto code={
          },
          lineto code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
          curveto code={
            \path [#1] (\tikzinputsegmentfirst)
            .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..
            (\tikzinputsegmentlast);
          },
          closepath code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
        },
      },
    %
    vector/.style={line join=round, line cap=round, thick, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start up}},
    %
    vector2/.style={line join=round, line cap=round, thick, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start down}},
    %
    gluon/.style={line join=round, line cap=round, thick, decorate, decoration={spring, amplitude=0.1*\tikz@node@distance, segment length=0.2*\tikz@node@distance, aspect=0.75}},
    %
    qline/.style={
        line join=round,
        line cap=round,
        thick,
        postaction={
            on each segment={
                decorate,
                decoration={
                    markings,
                    mark=at position 0.5*\pgfdecoratedpathlength+0.08*\tikz@node@distance with \arrow{Stealth[length=0.16*\tikz@node@distance, width=0.14*\tikz@node@distance]}
                }
            }
        }
    },
    tline/.style={
        qline,
        very thick
    },
    %
    higgs/.style={
        line join=round,
        line cap=round,
        thick,
        dashed
    }
}


\newcommand\myaction{}

\newcommand{\DrellYan}[4]{\tikz[node distance=#3, baseline=#4]
    {
    \draw [qline] (0,0) -- ++(-45:{sqrt(2)*#3}) coordinate (Vq) -- ++(-135:{sqrt(2)*#3});
    \draw [vector] (Vq) -- ++(0:0.85*#3) coordinate (VH) node [midway, above, yshift=0.15*#3] {$V^{\ast}$};
    \draw [vector] (VH) -- ++(45:0.85*#3) coordinate (Vl) node [midway, above, xshift=-0.2*#3, yshift=0.1*#3] {$V^{\ast}$};
    \draw [higgs] (VH) -- ++(-45:0.85*#3) coordinate (Hb) node [midway, below, xshift=-0.2*#3] {$\mathrm{H}$};
    \draw [qline] (Vl)++(67.5:0.75*#3) node [above,xshift=0.1*#3] (lb) {$\bar{\ell}$} -- (Vl) -- ++(22.5:0.75*#3) node [right, yshift=0.05*#3] (lb) {$\ell$};
    \draw [qline] (Hb)++(5:0.75*#3) node [right] (bb) {$\mathrm{\bar{b}}$} -- (Hb) -- ++(-95:0.75*#3) node [below] (b) {$\mathrm{b}$} ;

    % Draw gluon for production if #1 is 1
    \path (Vq)++(135:#3) coordinate (qg);
    \path \pgfextra{\ifthenelse{\equal{#1}{1}}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg) -- ++(22.5:#3);

    % Draw gluon for decay if #2 is 1
    \path (Hb)++(-95:0.2*#3) coordinate (bg);
    \path \pgfextra{\ifthenelse{\equal{#2}{1}}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (bg) -- ++(-30:0.8*#3);
    }
}


\newcommand{\ProdAnt}[2]{\tikz[node distance=#2]
    {
    \useasboundingbox (-0.2*#2,-2.2*#2) rectangle (2.2*#2,0.2*#2);
    \draw [qline] (0,0) -- ++(-45:{sqrt(2)*#2}) coordinate (Vq) -- ++(-135:{sqrt(2)*#2});
    \draw [vector] (Vq) -- ++(0:#2);

    % Draw gluon into the antenna when #1 is 1
    \path (Vq)++(135:#2) coordinate (qg);
    \path \pgfextra{\ifthenelse{\equal{#1}{1}}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg) -- ++(22.5:#2);
    }
}

\newcommand{\DecAnt}[2]{\tikz[node distance=#2]
    {
    \useasboundingbox (-0.2*#2,-1.2*#2) rectangle (2.2*#2, 1.2*#2);
    \draw [higgs] (0,0) -- ++(0:#2) coordinate (Hb);
    \draw [qline] (Hb)++(45:{sqrt(2)*#2}) -- (Hb) -- ++(-45:{sqrt(2)*#2});

    % Draw gluon into the antenna when #1 is 1
    \path (Hb)++(-45:0.3*#2) coordinate (bg);
    \path \pgfextra{\ifthenelse{\equal{#1}{1}}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (bg) -- ++(15:#2);
    }
}

\newcommand{\TopVII}[2]{\tikz[node distance=#1, baseline=#2]
    {
    \draw [qline] (0,0) -- ++(0:#1) coordinate (qg1) -- ++(-90:#1) coordinate (qg2) -- ++(180:#1);
    \draw [gluon] (qg1) -- ++(0:#1) coordinate (tg1);
    \draw [gluon] (qg2) -- ++(0:#1) coordinate (tg2);
    \draw [tline] (tg2) -- (tg1) -- ++(0:#1) coordinate (tV) -- ++(-90:#1) coordinate (tH) -- cycle;
    \draw [vector] (tV) -- ++(0:#1);
    \draw [higgs] (tH) -- ++(0:#1);
    }
}


\newcommand{\TopRII}[2]{\tikz[thick, node distance=#1, baseline=#2]
    {
    \draw [qline] (0,0) -- ++(-45:#1) coordinate (qg) -- ++(-135:#1);
    \draw [gluon] (qg) -- ++(0:#1) coordinate (tg1);
    \draw [tline] (tg1) -- ++(45:#1) coordinate (tV) -- ++(-45:#1) coordinate (tg2) -- ++ (-135:#1) coordinate (tH) -- cycle;
    \draw [vector2] (tV) -- ++(0:#1);
    \draw [gluon] (tg2) -- ++(0:#1);
    \draw [higgs] (tH) -- ++(0:#1);
    }
}


\newcommand{\TopVI}[2]{\tikz[node distance=#1, baseline=#2]
    {
    \draw [qline] (0,0) -- ++(-45:{sqrt(2)*#1}) coordinate (qV) -- ++(-135:{sqrt(2)*#1});
    \coordinate [above left=of qV] (qg1);
    \coordinate [below left=of qV] (qg2);
    \coordinate [left=of qV] (tcent);
    \def\Radius{0.5*(sqrt(2)-1)*#1}
    \def\AngleU{{180-2*asin(0.25*(sqrt(2)-1))}}
    \def\AngleD{{180+2*asin(0.25*(sqrt(2)-1))}}
    \path (qg2) arc (225:\AngleD:#1) coordinate (tg2) arc (\AngleD:\AngleU:#1) coordinate (tg1);
    \draw [gluon] (qg2) arc (225:\AngleD:#1);
    \draw [gluon] (tg1) arc (\AngleU:135:#1);
    \draw [line width=0.04*\tikz@node@distance] (tcent) circle (\Radius);
    \coordinate [above=\Radius of tcent, xshift={0.97*\Radius}] (t1);
    \coordinate [below=\Radius of tcent, xshift={-0.97*\Radius}] (t2);
    \path [tline] (t1) -- ++(-90:{2*\Radius});
    \path [tline] (t2) -- ++(90:{2*\Radius});
    \draw [vector] (qV) -- ++(0:#1) coordinate (tV);
    \path (tg2) arc (-90:-45:{\Radius}) coordinate (tH);
    \draw [higgs] (tH) -- ($(tV) - (0,0.75*#1)$);
    }
}


\newcommand{\TopRI}[2]{\tikz[node distance=#1, baseline=#2]
    {
    \draw [qline] (0,0) -- ++(0:#1) coordinate (qV) -- ++(-90:#1) coordinate (qg) -- ++(180:#1);
    \draw [vector] (qV) -- ++(0:#1);
    \draw [gluon] (qg) -- ++(0:#1) coordinate (g1t);
    \draw [tline] (g1t) -- ++(30:0.75*#1) coordinate (g2t) -- ++(-90:0.75*#1) coordinate (Ht) -- (g1t);
    \draw [gluon] (g2t) -- ++(0:#1);
    \draw [higgs] (Ht) -- ++(0:#1);
    }
}

\newcommand{\TopSelfZHI}[2]{\tikz[node distance=#1, baseline=#2]
    {
    \draw [gluon] (0,0) -- ++(0:#1) coordinate (g1t);
    \draw [tline] (g1t) -- ++(0:#1) coordinate (tV) -- ++(-90:#1) coordinate (tH) -- ++(0:-#1) coordinate (g2t) -- (g1t);
    \draw [gluon] (g2t) -- ++(0:-#1);
    \draw [higgs] (tH) -- ++(0:#1);
    \draw [vector2] (tV) -- ++(0:#1);
    }
}


\newcommand{\TopSelfZHII}[2]{\tikz[node distance=#1, baseline=#2]
    {
    \draw [gluon] (0,0) -- ++(0:#1) coordinate (g1t);
    \draw [tline] (g1t) -- ++(-30:#1) coordinate (tV) -- ++(-150:#1) coordinate (g2t) -- (g1t);
    \draw [gluon] (g2t) -- ++(0:-#1);
    \draw [vector] (tV) -- ++(0:#1) coordinate (tH);
    \draw [vector] (tH) -- ++(45:#1);
    \draw [higgs] (tH) -- ++(-45:#1);
    }
}

\newcommand{\VHjets}[3]{\tikz[node distance=#2, baseline=#3]
    {
    \def\angle{10}
    \draw [thick, decoration={markings, mark=at position 0.6 with \arrow{latex}},postaction=decorate] (0,0) -- ++(-45:{sqrt(2)*#2}) coordinate (VH);
    \draw [thick, decoration={markings, mark=at position 0.6 with \arrow{latex}},postaction=decorate] (VH)++(-135:{sqrt(2)*#2}) -- (VH);
    \draw [vector] (VH) -- ++(30:#2) coordinate (V);
    \draw [higgs] (VH) -- ++(-30:#2) coordinate (H);
    \draw [qline] (V)++(60:#2) node [above right] (lb) {\small $\bar{\ell\,}$} -- (V) -- ++(20:#2) node [right] (l) {\small $\ell$};

    \draw [qline,red] (H)++(-20:#2) node [right] (bb) {\small $\mathrm{b}$-jet} -- (H) -- ++(-60:#2) node [below] (b) {\small $\mathrm{b}$-jet};
    \begin{scope}[rotate around={-20:(H)}]
      \draw [red] (H)++(\angle:#2) -- (H) -- ++(-\angle:#2);
      \draw [red] (H)++({cos(\angle)*#2},0) circle ({0.5*sin(\angle)*#2} and {sin(\angle)*#2});
    \end{scope}
    \begin{scope}[rotate around={-60:(H)}]
      \draw [red] (H)++(\angle:#2) -- (H) -- ++(-\angle:#2);
      \draw [red] (H)++({cos(\angle)*#2},0) circle ({0.5*sin(\angle)*#2} and {sin(\angle)*#2});
    \end{scope}

    \pgfextra{\ifthenelse{\equal{#1}{1}}{
        \path (H)++(20:#2) node [right] (j1) {\small light/$\mathrm{b}$-jet};
        \begin{scope}[rotate around={20:(H)}]
          \draw (H)++(\angle:#2) -- (H) -- ++(-\angle:#2);
          \draw (H)++({cos(\angle)*#2},0) circle ({0.5*sin(\angle)*#2} and {sin(\angle)*#2});
        \end{scope}
        \path (VH)++(-90:#2) node [below] (j1) {\small light/$\mathrm{b}$-jet};
        \begin{scope}[rotate around={-90:(VH)}]
          \draw (VH)++(\angle:#2) -- (VH) -- ++(-\angle:#2);
          \draw (VH)++({cos(\angle)*#2},0) circle ({0.5*sin(\angle)*#2} and {sin(\angle)*#2});
        \end{scope}
    }{}} % end pgfextra ifthenelse

    \filldraw [draw=white] (VH) circle [radius=0.1*#2];
    \filldraw [draw=white] (H) circle [radius=0.1*#2];
    }
}

\newcommand\mycolor{black}
\newcommand{\NaiveAntiKT}[3]{\tikz[node distance=#1, baseline=#2]
    {
    \def\angle{20}

    \pgfextra{\ifthenelse{\equal{#3}{1}}{
        \renewcommand\mycolor{red}
        \draw [ultra thick, line cap=round, red] (0,0) -- ++(135:0.3*#1);
        \draw [ultra thick, line cap=round, red] (0,0) -- ++(5:0.3*#1);
        }{
        \draw [thick, line cap=round, decorate, decoration={spring, amplitude=0.05*\tikz@node@distance, segment length=0.1*\tikz@node@distance, aspect=0.75}] (0,0) -- ++(70:0.4*#1);
        }

        \begin{scope}[rotate around={140:(0,0)}]
            \draw [\mycolor] (0,0)++(\angle:#1) -- (0,0) -- ++(-\angle:#1);
            \draw [\mycolor] (0,0)++({cos(\angle)*#1},0) circle ({0.5*sin(\angle)*#1} and {sin(\angle)*#1});
        \end{scope}

        \begin{scope}[rotate around={10:(0,0)}]
            \draw [\mycolor] (0,0)++(\angle:#1) -- (0,0) -- ++(-\angle:#1);;
            \draw [\mycolor] (0,0)++({cos(\angle)*#1},0) circle ({0.5*sin(\angle)*#1} and {sin(\angle)*#1});
        \end{scope}
        \filldraw [draw=white] (0,0) circle [radius=0.1*#1];
    } % pgfextra closing bracket

    \begin{scope}[rotate around={-90:(0,0)}]
        \draw (0,0)++(\angle:0.7*#1) -- (0,0) -- ++(-\angle:0.7*#1);;
        \draw (0,0)++({cos(\angle)*0.7*#1},0) circle ({0.5*sin(\angle)*0.7*#1} and {sin(\angle)*0.7*#1});
    \end{scope}

    } % tikz closing bracket
}

\makeatother

